From the Quantum Approximate Optimization Algorithm to a Quantum Alternating Operator Ansatz

The next few years will be exciting as prototype universal quantum processors emerge, enabling implementation of a wider variety of algorithms. Of particular interest are quantum heuristics, which require experimentation on quantum hardware for their evaluation, and which have the potential to significantly expand the breadth of quantum computing applications. A leading candidate is Farhi et al.'s Quantum Approximate Optimization Algorithm, which alternates between applying a cost-function-based Hamiltonian and a mixing Hamiltonian. Here, we extend this framework to allow alternation between more general families of operators. The essence of this extension, the Quantum Alternating Operator Ansatz, is the consideration of general parametrized families of unitaries rather than only those corresponding to the time-evolution under a fixed local Hamiltonian for a time specified by the parameter. This ansatz supports the representation of a larger, and potentially more useful, set of states than the original formulation, with potential long-term impact on a broad array of application areas. For cases that call for mixing only within a desired subspace, refocusing on unitaries rather than Hamiltonians enables more efficiently implementable mixers than was possible in the original framework. Such mixers are particularly useful for optimization problems with hard constraints that must always be satisfied, defining a feasible subspace, and soft constraints whose violation we wish to minimize. More efficient implementation enables earlier experimental exploration of an alternating operator approach to a wide variety of approximate optimization, exact optimization, and sampling problems. Here, we introduce the Quantum Alternating Operator Ansatz, lay out design criteria for mixing operators, detail mappings for eight problems, and provide brief descriptions of mappings for diverse problems.

==> macros.tex <==
% For easy commenting
\definecolor{nblue}{rgb}{0.3,0.3,1.0}%229
\definecolor{ngreen}{rgb}{0.2,0.7,0.2}%161
\definecolor{nred}{rgb}{0.9,0.1,0}%711&900
\definecolor{nmagenta}{rgb}{255,0,255}%711&900
\definecolor{nviol}{rgb}{0.7,0.1,0.7}
\newcommand{\blu}{\color{nblue}}
\newcommand{\vio}{\color{violet}}
\newcommand{\grn}{\color{ngreen}}
\newcommand{\red}{\color{nred}}
\newcommand{\blk}{\color{black}}
\newcommand{\egr}[1]{{\color{nblue} \small \bf [[{#1}]]}}
\newcommand{\sh}[1]{{\color{ngreen} \small \bf [[{#1}]]}}
\newcommand{\magenta}[1]{{\color{nmagenta}#1}}
\newcommand{\viol}[1]{{\color{nviol}#1}}
\newcommand{\redtext}[1]{{\color{nred}#1}}

\newcommand{\ea}{et al.}
\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }

\newcommand{\B}{{\{0, 1\}}}

\newcommand{\hc}{\mathrm{h.c.}}

\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\w}{\mathbf{w}}

\newcommand{\e}{\epsilon}

\newcommand{\bqa}{\begin{eqnarray}}
\newcommand{\eqa}{\end{eqnarray}}
\newcommand{\ketbra}[2]{\ket{#1}\!\bra{#2}}

\newcommand{\tikzmark}[1]{\tikz[overlay,remember picture] \node (#1) {};}


==> notation.tex <==
\newcommand{\reals}{{\mathbb{R}}}
\newcommand{\integers}{{\mathbb{Z}}}
\newcommand{\complexes}{{\mathbb{C}}}
\newcommand{\naturals}{{\mathbb{N}}}

\newcommand{\colorParity}{\mathrm{CP}}
\newcommand{\timeParity}{\mathrm{TP}}


\newcommand{\OPT}{\mathrm{OPT}}

% ansatz 
\newcommand{\QAOA}{\mathrm{QAOA}} % class of circuits of this form, as well as algorithm name
\newcommand{\QAOAcirc}{Q} % For unitary from a full QAOA circuit, the product of 2p ops.
\newcommand{\domain}{F}
\newcommand{\domainQ}{\mathcal{F}}
\newcommand{\objFunc}{f}
\newcommand{\objHam}{H_{\objFunc}}
\newcommand{\objUnitary}{U_{\objFunc}}
\newcommand{\phaseFunc}{g}
\newcommand{\phaseHam}{H_{\mathrm{P}}}
\newcommand{\mixHam}{H_{\mathrm{M}}}
\newcommand{\mixUnitary}{U_{\mathrm{M}}}
\newcommand{\stdDriver}{H_B}
\newcommand{\initial}{s}
\newcommand{\iniState}{\ket{\initial}}
\newcommand{\hamDist}{\mathrm{Ham}}

\newcommand\phaseUnitary[1][]{
  \ifstrempty{#1}{
    U_{\mathrm{P}}
  }{
    U_{\mathrm{P},#1}
  }
}


\newcommand\Ham[2][]{
  \ifstrempty{#1}{
    H_{#2}
  }{
    H_{#1, #2}
  }
}

\newcommand\unitary[2][]{
  \ifstrempty{#1}{
    U_{#2}
  }{
    U_{#1, #2}
  }
}

\newcommand{\rnv}[1][r]{#1\text{-}\mathrm{NV}}
\newcommand{\ring}{\mathrm{ring}}
\newcommand{\fc}{\mathrm{FC}}

\newcommand{\timeEv}[1]{e^{-i #1}}
\newcommand{\comp}{(\mathrm{comp})}
\newcommand{\enc}{(\mathrm{enc})}
\newcommand{\parity}{\mathrm{parity}}
\newcommand{\even}{\mathrm{even}}
\newcommand{\odd}{\mathrm{odd}}
\newcommand{\last}{\mathrm{last}}
\newcommand{\identity}{I}
\newcommand{\quditSwap}{\mathrm{XY}}
\newcommand{\binary}{\mathrm{binary}}
\newcommand{\controlX}{\mathrm{CX}}
\newcommand{\control}{\Lambda}

\newcommand{\controlFunc}{\chi}
\newcommand{\proj}{H_{\controlFunc}}

\newcommand{\simMixer}[1]{\mathrm{sim}\text{-}#1}
\newcommand{\seqMixer}[1]{\mathcal{P}\text{-}#1}
\newcommand{\simCX}{\simMixer{\controlX}}
\newcommand{\seqCX}{\seqMixer{\controlX}}

\newcommand{\add}{\mathrm{ADD}}

\newcommand{\controlXY}{\mathrm{CXY}}

\newcommand{\nullSwap}{\mathrm{NS}}
\newcommand{\simNullSwap}{\simMixer{\nullSwap}}
\newcommand{\seqNullSwap}{\seqMixer{\nullSwap}}
\newcommand{\controlSwap}{\mathrm{CS}}
\newcommand{\simControlSwap}{\simMixer{\nullSwap}}
\newcommand{\seqControlSwap}{\seqMixer{\nullSwap}}
\newcommand{\permSwap}{\mathrm{PS}}
\newcommand{\simPermSwap}{\simMixer{\permSwap}}
\newcommand{\seqPermSwap}{\seqMixer{\permSwap}}
\newcommand{\timeSwap}{\mathrm{TS}}
\newcommand{\timeColor}{\mathrm{TC}}

\newcommand{\charSwap}{\mathrm{CS}}
\newcommand{\NONE}{\mathsf{NONE}}

% general problem specification
\newcommand{\neighborFunc}{\mathrm{nbhd}}
% \newcommand{\neighborFunc}{\mathrm{nbd}} %nbhd is commonly used in the math community. I (EGR) have never seen nbd.
\newcommand{\quditDim}{d}
\newcommand{\arity}{k}
\newcommand{\numVars}{n}
\newcommand{\numConstraints}{m}
\newcommand{\perm}{\boldsymbol{\sigma}}
\newcommand{\permElmt}{\sigma}
\newcommand{\invPerm}{\perm^{-1}}
\newcommand{\invPermElmt}{\permElmt^{-1}}
\newcommand{\perms}{\Sigma}
\newcommand{\order}{\boldsymbol{\iota}}
\newcommand{\orderElmt}{\iota}

\newcommand{\graphComp}[1]{\overline{#1}}

\newcommand{\create}{S^{+}}
\newcommand{\annihilate}{S^{-}}

% graphs
\newcommand{\numColors}{\kappa}
\newcommand{\degree}{D}
\newcommand{\distance}{d}

% scheduling
\newcommand{\strtTime}{s}
\newcommand{\strtTimes}{\mathbf{s}}
\newcommand{\lastStrtTime}{h}
\newcommand{\releaseTime}{r}
\newcommand{\releaseTimes}{\mathbf{r}}
\newcommand{\window}{W}
\newcommand{\deadline}{d}
\newcommand{\deadlines}{\mathbf{\deadline}}
\newcommand{\weight}{w}
\newcommand{\weights}{\mathbf{w}}
\newcommand{\procTime}{p}
\newcommand{\procTimes}{\mathbf{\procTime}}
\newcommand{\horizon}{h}

% logic
\newcommand{\NEQ}{\mathsf{NEQ}}
\newcommand{\EQ}{\mathsf{EQ}}
\newcommand{\NOR}{\mathsf{NOR}}
\newcommand{\OR}{\mathsf{OR}}
\newcommand{\AND}{\mathsf{AND}}

\newcommand\allNeighbors[2][]{
  \ifstrempty{#1}{
    \AND(x_{\neighborFunc(#2)})
  }{
    \AND(x_{\neighborFunc(#1), #2})
  }
}

\newcommand\noNeighbors[2][]{
  \ifstrempty{#1}{
    \NOR(x_{\neighborFunc(#2)})
  }{
    \NOR(x_{\neighborFunc(#1), #2})
  }
}

% qudits
\newcommand{\quditX}{{\breve{X}}}
\newcommand{\quditZ}{{\breve{Z}}}

% operators
\newcommand{\SWAP}{\mathrm{SWAP}}
\newcommand{\XYij}{X_iX_j+Y_iY_j}
\newcommand{\SWAPij}{\SWAP_{i,j}}

